Enhancing Graph Contrastive Learning with Reliable and Informative Augmentation for Recommendation

Graph neural network(GNN) has been a powerful approach in collaborative filtering(CF) due to its ability to model high-order user-item relationships. Recently, to alleviate the data sparsity and enhance representation learning, many efforts have been conducted to integrate contrastive learning(CL) with GNNs. Despite the promising improvements, the contrastive view generation based on structure and representation perturbations in existing methods potentially disrupts the collaborative information in contrastive views, resulting in limited effectiveness of positive alignment. To overcome this issue, we propose CoGCL, a novel framework that aims to enhance graph contrastive learning by constructing contrastive views with stronger collaborative information via discrete codes. The core idea is to map users and items into discrete codes rich in collaborative information for reliable and informative contrastive view generation. To this end, we initially introduce a multi-level vector quantizer in an end-to-end manner to quantize user and item representations into discrete codes. Based on these discrete codes, we enhance the collaborative information of contrastive views by considering neighborhood structure and semantic relevance respectively. For neighborhood structure, we propose virtual neighbor augmentation by treating discrete codes as virtual neighbors, which expands an observed user-item interaction into multiple edges involving discrete codes. Regarding semantic relevance, we identify similar users/items based on shared discrete codes and interaction targets to generate the semantically relevant view. Through these strategies, we construct contrastive views with stronger collaborative information and develop a triple-view graph contrastive learning approach. Extensive experiments on four public datasets demonstrate the effectiveness of our proposed approach.

==> sec_methodology_bak.tex <==
\section{Methodology}

In this section, we present our proposed XXX, which ...


\subsection{Approach Overview}

As outlined in Sections~\ref{sec:intro} and~\ref{sec:preliminary}, we are motivated by the potential of graph contrastive learning for local clustering in collaborative filtering, rather than emphasizing global uniformity as in previous works.
In this context, we anticipate that the positive pairs align with the principle of collaborative similarity, which is demonstrated in two aspects: \emph{common neighbors on the graph structure} or \emph{semantic similarity learned by GNN}.
Inspired by recent studies~\cite{DBLP:conf/www/HouHMZ23,DBLP:conf/nips/RajputMSKVHHT0S23,DBLP:journals/corr/abs-2311-09049} on user/item ID discretization in recommender systems, we innovatively employ discrete IDs (called \emph{codes} to distinguish from the vanilla ID) for virtual neighbor augmentation and semantic similarity discrimination.
Specifically, our framework contains two types of positive pairs:

\begin{itemize}
    \item \textbf{Graphs augmented by virtual neighbors}: We learn an additional identifier for each user/item alongside the vanilla ID, which consists of a tuple of discrete codes that imply collaborative semantics.
    Utilizing these codes, we augment the graph structure by replacing node neighbors in the graph with their codes or directly adding codes as virtual neighbors.
    The resulting graphs, following two rounds of augmentation, are considered positive pairs due to the substantial overlap of common neighbors between identical nodes.
    \item \textbf{Users/Items with similar collaborative relationships}: 
    Given that shared discrete codes signify semantic similarity between users/items, we regard those with multiple shared codes as positive instances. Furthermore, users/items with common interactions are also considered similar.
\end{itemize}

The overall framework of our proposed approach is illustrated in Figure~\ref{fig:model}. 
Firstly, we introduce the methodology for learning discrete codes for users/items and their application in virtual neighbor augmentation~(Section~\ref{sec:code_aug}). Secondly, we present the GNN architecture employed in our framework~(Section~\ref{sec:gnn}).
Finally, we elaborate on the procedure of triple-view contrastive learning, focusing on the alignment between two graph augmentation views and the similar user/item view~(Section~\ref{sec:cl}).





\subsection{User/Item as Multiple Discrete Codes}
\label{sec:code_aug}
In this section, we begin by introducing how to learn semantically related discrete codes for users and items within our framework. Subsequently, we delve into the method for graph augmentation using the learned discrete codes.


\subsubsection{Discrete Codes Learning}

Common approaches to learning semantically related discrete codes include hierarchical clustering~\cite{DBLP:journals/widm/MurtaghC12，DBLP:journals/corr/abs-2309-13375}, semantic hashing~\cite{DBLP:conf/stoc/Charikar02}, and vector quantization~\cite{gray1984vector,DBLP:conf/nips/RajputMSKVHHT0S23}. Our approach adopts the multi-level vector quantization method that can be learned end-to-end, such as residual quantization~(RQ)~\cite{DBLP:journals/sensors/ChenGW10} and product quantization~(PQ)~\cite{DBLP:journals/pami/JegouDS11}.
We take discrete codes of users as an example to introduce the learning process, and item codes can be obtained analogously.
At each level $h$, there exists a codebook $\mathcal{C}^h = \{\mathbf{e}_k^h\}_{k=1}^K$, where each vector $\mathbf{e}_k^h$ is a learnable cluster center. Then the quantization process can be expressed as:
\begin{align}
    & c_u^h = \underset {k} { \operatorname {arg\,min} } \ g(\mathbf{z}_u^h, \mathbf{e}_k^h) , 
    \label{eq:vq}
\end{align}
where $c_u^h$ is the $h$-th code for the user, $\mathbf{z}_u^h$ denotes user representation at the $h$-th level, and $g(\cdot)$ is distance function~(\eg, euclidean distance and cosine distance).
Given the user representation $\mathbf{z}_u$ readout from GNN in Eq.~\eqref{eq:gnn}, RQ calculates residuals as representations for each level, denoted by $\mathbf{z}_u^{h+1} = \mathbf{z}_u^h - \mathbf{e}_{c_h}^h$, and $\mathbf{z}_u^1 = \mathbf{z}_u$.
PQ splits $\mathbf{z}_u$ into $H$ sub-vectors $\mathbf{z}_u = \left[\mathbf{z}_u^1;\dots, \mathbf{z}_u^H  \right]$, each of dimension $d/H$, where H is the total number of levels.




\subsubsection{Graph Augmentation via Discrete Codes}
Given the learned discrete codes for users and items, we further utilize them to augment node neighbors in the interaction graph. Taking user $u$ as an example, we first randomly sample from his/her neighbors $\mathcal{N}_u$ with probability $p$ for data augmentation. Then we divide the sampled neighbors into two groups $\mathcal{N}_u^{r}$ and $\mathcal{N}_u^{a}$ for ``Replace'' and ``Add'' augmentation respectively. 
The former replaces the neighbor items with their corresponding codes, which means that the original edges are not retained, while the latter directly adds the codes as virtual neighbors. Formally, the augmented edge of $u$ can be expressed as:
% \begin{align}
%     \mathcal{E}_u^{r} &= \left\{(u,c_i^{h})| i \in \mathcal{N}_u^{r}, h \in \{1,\dots,H\}\right\}, \\
%     \mathcal{E}_u^{a} &= \left\{(u,c_i^{h})| i \in \mathcal{N}_u^{a}, h \in \{1,\dots,H\}\right\} \cup \left\{(u,i)| i \in \mathcal{N}_u^{a}\right\}, \\
%     \mathcal{E}_u^{\prime} &=  \left\{(u,i)| i \in \mathcal{N}_u \setminus (\mathcal{N}_u^{r} \cup \mathcal{N}_u^{a}) \right\} \cup \mathcal{E}_u^{r} \cup \mathcal{E}_u^{a},
% \end{align}
\begin{align}
    \mathcal{E}_u^{c} &= \left\{(u,c_i^{h})| i \in (\mathcal{N}_u^{r} \cup \mathcal{N}_u^{a}), h \in \{1,\dots,H\}\right\}, \\
    \mathcal{E}_u^{\prime} &=  \left\{(u,i)| i \in (\mathcal{N}_u \setminus \mathcal{N}_u^{r}) \right\} \cup \mathcal{E}_u^{c},
\end{align}
where $\mathcal{E}_u^{c}$ denotes the edges between user $u$ and discrete codes, $\mathcal{E}_u^{\prime}$ is all interaction edges of the user after augmentation. 
In this case, discrete codes can be regarded as virtual neighbors of the user. 
Moreover, the operations described above, which entail either replacing the original edges with multiple edges or directly adding extra edges, can effectively alleviate the sparsity of the graph. 
The graph augmentation for items can be symmetrically performed.
In order to construct different views of the graph, we randomly perform two rounds of graph augmentation. The augmented graph is depicted as follows:
\begin{align}
    \mathcal{G}^{\prime}=(\widetilde{\mathcal{V}}, \mathcal{E}^{\prime}), \ \ \ \ \ 
    \mathcal{G}^{\prime\prime}=(\widetilde{\mathcal{V}}, \mathcal{E}^{\prime\prime})
\end{align}
where the node set $\widetilde{\mathcal{V}}=\{\mathcal{U} \cup \mathcal{C}^U  \cup \mathcal{I} \cup \mathcal{C}^I\}$ comprises all users, items and their corresponding discrete codes. $\mathcal{E}^{\prime}$ and $\mathcal{E}^{\prime\prime}$ denote the edge sets resulting from the aforementioned virtual neighbor augmentation for all users and items.

\subsection{Multi-View Representation Modeling via GNN}
\label{sec:gnn}


\subsection{Triple View Graph Contrastive Learning}
\label{sec:cl}


\subsubsection{Augmented Graph Contrast}


\subsubsection{Similar User/Item Contrast}



\subsubsection{Overall Optimization}


\subsection{Discussion}
